Ultrasound Video Summarization using Deep Reinforcement Learning

Video is an essential imaging modality for diagnostics, e.g. in ultrasound imaging, for endoscopy, or movement assessment. However, video hasn't received a lot of attention in the medical image analysis community. In the clinical practice, it is challenging to utilise raw diagnostic video data efficiently as video data takes a long time to process, annotate or audit. In this paper we introduce a novel, fully automatic video summarization method that is tailored to the needs of medical video data. Our approach is framed as reinforcement learning problem and produces agents focusing on the preservation of important diagnostic information. We evaluate our method on videos from fetal ultrasound screening, where commonly only a small amount of the recorded data is used diagnostically. We show that our method is superior to alternative video summarization methods and that it preserves essential information required by clinical diagnostic standards.

==> related_work.tex <==
Video summarization based tele-endoscopy: a service to efficiently manage visual data generated during wireless capsule endoscopy procedure

==> table.tex <==
% %-----------------------------------------------------------

\begin{table}[htb]
\center
\begin{tabular}{ccccc}
\multicolumn{3}{c|}{Rewards} &
\multicolumn{2}{c|}{Learning paradigm} \\
\toprule
$\mathcal{R}_{\text {rep}}$ &  
$\mathcal{R}_{\text {div}}$  & 
$\mathcal{R}_{\text {det}}$  & 
Unsupervised & 
Supervised   \\ 
\hline
$\times$   &  
$\times$   &   
$\times$   &   
-   &      
xxx   \\ 
% \cline{2-5}
\checkmark &  
$\times$  &   
$\times$   &   
xxx   &   
\textbf{xx}       \\ 
% \cline{2-5} 
$\times$      & 
$\times$   &   
\checkmark &   
xxx   &       
xxx      \\ 
% \cline{2-5} 
\checkmark & 
\checkmark &    
$\times$   &   
\textbf{xx}     &      
xxx         \\ 
\checkmark & 
\checkmark &    
\checkmark &
\textbf{xx}     &      
xxx         \\ 
\checkmark & 
\checkmark &    
\checkmark &
\textbf{xx}     &      
xxx        \\ 
\checkmark & 
\checkmark &    
\checkmark &
\textbf{xx}     &      
xx         \\ 
\bottomrule
\end{tabular}
\caption{F1 scores  using an unsupervised and a supervised learning paradigm with or ($\times$) without ($\checkmark$) $\mathcal{R}_{\text {rep}}$ and $\mathcal{R}_{\text {div}}$ reward terms. Best score in bold.}
\label{tab:w_o_award}
\vspace{-10mm}
\end{table}

%By using RL for video summarization, the action on selecting a frame in the summary can be taken inter-dependently so that the selection of one frame would have implications on the selection of others. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{lllllllll}
\multicolumn{3}{l}{Rewards}    & \multicolumn{6}{l}{Learning paradigm}    \\
\multirow{2}{*}{R1} & \multirow{2}{*}{R2} & \multirow{2}{*}{R3} & \multicolumn{3}{r}{unsupervised} & \multicolumn{3}{l}{supervised} \\
         &          &          & F                    & P & R & F & P & R \\
$\times$ & $\times$ & $\times$ & \multicolumn{1}{r}{} &   &   &   &   &   \\
y        & $\times$ & $\times$ & \multicolumn{1}{r}{} &   &   &   &   &   \\
x        & y        & $\times$ & \multicolumn{1}{r}{} &   &   &   &   &   \\
y        & y        & $\times$ &                      &   &   &   &   &   \\
$\times$ & $\times$ & y        &                      &   &   &   &   &   \\
y        & $\times$ & y        &                      &   &   &   &   &   \\
$\times$ & y        & y        &                      &   &   &   &   &   \\
y        & y        & y        &                      &   &   &   &   &  
\end{tabular}
\end{table}

%-------------------------------------
 %-----------------------------------------------------------
\begin{table}[htb]
\center
\begin{tabular}{ccccc}
\multicolumn{3}{c|}{Rewards} &
\multicolumn{2}{c|}{Learning paradigm} \\
\toprule
$\mathcal{R}_{\text {rep}}$ &  
$\mathcal{R}_{\text {div}}$  & 
$\mathcal{R}_{\text {det}}$  & 
Unsupervised & 
Supervised   \\ 
\hline
$\times$   &  
$\times$   &   
$\times$   &   
-   &      
xxx   \\ 
% \cline{2-5}
\checkmark &  
$\times$  &   
$\times$   &   
xxx   &   
\textbf{xx}       \\ 
% \cline{2-5} 
$\times$      & 
$\times$   &   
\checkmark &   
xxx   &       
xxx      \\ 
% \cline{2-5} 
\checkmark & 
\checkmark &    
$\times$   &   
\textbf{xx}     &      
xxx         \\ 
\checkmark & 
\checkmark &    
\checkmark &
\textbf{xx}     &      
xxx         \\ 
\checkmark & 
\checkmark &    
\checkmark &
\textbf{xx}     &      
xxx        \\ 
\checkmark & 
\checkmark &    
\checkmark &
\textbf{xx}     &      
xx         \\ 
\bottomrule
\end{tabular}
\caption{F1 scores  using an unsupervised and a supervised learning paradigm with or ($\times$) without ($\checkmark$) $\mathcal{R}_{\text {rep}}$ and $\mathcal{R}_{\text {div}}$ reward terms. Best score in bold.}
\label{tab:w_o_award}
\vspace{-10mm}
\end{table}

% %-----------------------------------------------------------
% \begin{table}[tp]
% \center
% \caption{Comparison to state-of-the-arts video summarization methods.}
% \setlength{\tabcolsep}{2.5mm}{
% \begin{tabular}{l|l|l|l|l|l|l}
% Methods        & split 1 &  split 2  & split 3  & split 4  & split 5 & Average \\ \hline
% FCSN_{sup}~\cite{FCSN_eccv2018}&  
% 58.24 & \textbf{61.51} & 57.08 & 59.48 & 59.54  & 59.17 \\ \hline
% DR-DSN_{sup}~\cite{RLvSumm_AAAI2018} &
% 57.34 & 58.97 & 60.63 & 62.43 & 61.16  & 60.34   \\ \hline
% Proposed_{sup}(our) & 
% \textbf{62.33} & 60.62  & \textbf{61.96} & \textbf{66.05} & \textbf{65.51} & \textbf{63.29}\\ 
%  \hline\hline
% %FCSN_{unsup}~\cite{FCSN_eccv2018}   & &   & &     & &\\ \hline
% DR-DSN_{unsup}~\cite{RLvSumm_AAAI2018}  & 40.92 & 39.48  & &   & &  \\ \hline
% Proposed_{unsup}(our)    &   59.58   & 52.86   &  56.74  & 57.25 & 57.20 & 56.73\\\hline
% \end{tabular}}
% \label{tab:SoA_comp}
% \end{table}
% %-----------------------------------------------------------

% %-----------------------------------------------------------
% \begin{table}[tp]
% %\center
% \caption{Comparison to state-of-the-arts video summarization methods.}
% \setlength{\tabcolsep}{2.5mm}{
% \begin{tabular}{l|l}
% Methods         & F1-scores\\ \hline
% FCSN_{sup}~\cite{FCSN_eccv2018}& 59.17 \\ \hline
% DR-DSN_{sup}~\cite{RLvSumm_AAAI2018}  & 60.34   \\ \hline
% Proposed_{sup}(our) & \textbf{63.29}\\ 
%  \hline\hline
% %FCSN_{unsup}~\cite{FCSN_eccv2018}   & &   & &     & &\\ \hline
% DR-DSN_{unsup}~\cite{RLvSumm_AAAI2018}  & 40.92  \\ \hline
% Proposed_{unsup}(our)    &   \textbf{56.73}\\\hline
% \end{tabular}}
% \label{tab:SoA_comp}
% \end{table}
% %-----------------------------------------------------------
% %-----------------------------------------------------------
% \begin{figure}[t]
% \begin{centering}
% \center\includegraphics[width=0.45\columnwidth]{images/ifind_propotion.png}
% \par\end{centering}
% \caption{xx}
% \label{fig:proportion}
% \end{figure}
% %-----------------------------------------------------------


% \begin{table}
% \begin{minipage}[b]{0.47\textwidth}
% \captionof{table}{Comparison to state-of-the-arts video summarization methods.}
% \begin{footnotesize}
% \centering%
% \setlength{\tabcolsep}{2.5mm}{
% \begin{tabular}{ l | c } \hline
% Methods         & F1-scores\\ \hline
% FCSN_{sup}~\cite{FCSN_eccv2018}& 59.17 \\ \hline
% DR-DSN_{sup}~\cite{RLvSumm_AAAI2018}  & 60.34   \\ \hline
% Proposed_{sup}(our) & \textbf{63.29}\\ 
%  \hline\hline
% %FCSN_{unsup}~\cite{FCSN_eccv2018}   & &   & &     & &\\ \hline
% DR-DSN_{unsup}~\cite{RLvSumm_AAAI2018}  & 40.92  \\ \hline
% Proposed_{unsup}(our)    &   \textbf{56.73}\\\hline
% \end{tabular}}
% \end{footnotesize}
% % \vspace{3.5mm}
% \label{tab:SoA_comp}
% \end{minipage}\hfill
% % \hspace{-1cm}
% \begin{minipage}[b]{0.48\textwidth}%
%  \centering
%   \includegraphics[width=0.9\columnwidth]{images/ifind_propotion.png}
%   \captionof{figure}{Figure 1}
%   \label{fig:proportion}
% \end{minipage}
% \end{table}

%TODO going to reshape this now

\iffalse
\begin{minipage}{\textwidth}
\begin{minipage}[b]{0.49\textwidth}
\centering
\begin{tabular}{ l | c } \hline
Methods         & F1-scores\\ \hline
FCSN_{sup}~\cite{FCSN_eccv2018}& 59.17 \\ \hline
DR-DSN_{sup}~\cite{RLvSumm_AAAI2018}  & 60.34   \\ \hline
Proposed_{sup}(our) & \textbf{63.29}\\ 
 \hline\hline
%FCSN_{unsup}~\cite{FCSN_eccv2018}   & &   & &     & &\\ \hline
DR-DSN_{unsup}~\cite{RLvSumm_AAAI2018}  & 40.92  \\ \hline
Proposed_{unsup}(our)    &   \textbf{56.73}\\\hline
\end{tabular}
%\end{footnotesize}
%\vspace{3.5mm}
%\caption{Comparison to state-of-the-art video summarization methods. Best results in bold.}
\label{tab:SoA_comp}
  \captionof{table}{Comparison to state-of-the-art video summarization methods. Best results in bold.}
\end{minipage}
\hfill
\begin{minipage}[b]{0.49\textwidth}
\centering
\includegraphics[width=0.9\columnwidth]{images/ifind_propotion.png}
\captionof{figure}{Performance of supervised vs. unsupervised summarization for different summary lengths.}
\end{minipage}
\end{minipage}
\fi

